Retrieval-Constrained Decoding Reveals Underestimated Parametric Knowledge in Language Models

Language models (LMs) encode substantial factual knowledge, but often produce answers judged as incorrect. We hypothesize that many of these answers are actually correct, but are expressed in alternative surface forms that are dismissed due to an overly strict evaluation, leading to an underestimation of models' parametric knowledge. We propose Retrieval-Constrained Decoding (RCD), a decoding strategy that restricts model outputs to unique surface forms. We introduce YAGO-QA, a dataset of 19,137 general knowledge questions. Evaluating open-source LMs from 135M to 70B parameters, we show that standard decoding undervalues their knowledge. For instance, Llama-3.1-70B scores only 32.3% F1 with vanilla decoding but 46.0% with RCD. Similarly, Llama-3.1-8B reaches 33.0% with RCD, outperforming the larger model under vanilla decoding. We publicly share the code and dataset at https://github.com/Rajjaa/disambiguated-LLM.

==> tables/YAGO_relations_mapping.tex <==
\begin{table}[]
    \centering
    \small
\begin{tabular}{lp{0.4\textwidth}}
\toprule
YAGO Relation & Wikidata Relation \\
\midrule
schema:award & award received \\
schema:author & author, creator \\
schema:contentLocation & narrative location \\
schema:inLanguage & language of work or name \\
schema:illustrator & illustrator \\
schema:editor & editor \\
schema:publisher & publisher \\
schema:sponsor & sponsor \\
schema:musicBy & composer \\
schema:actor & cast member \\
schema:locationCreated & country of origin, location of formation \\
schema:director & director \\
schema:productionCompany & production company \\
schema:lyricist & lyricist \\
yago:appearsIn & present in work, first appearance, from fictional universe \\
schema:performer & performer \\
schema:location & located in/on physical feature, location, located in the administrative territorial entity, mountain range, country \\
schema:organizer & organizer \\
yago:follows & follows \\
yago:participant & participating team, participant \\
schema:founder & founded by \\
yago:leader & head of state, head of government \\
schema:memberOf & member of \\
yago:ownedBy & owned by, parent organization \\
yago:notableWork & notable work \\
yago:influencedBy & inspired by, influenced by \\
yago:academicDegree & academic degree \\
schema:worksFor & employer \\
schema:alumniOf & educated at \\
schema:children & child \\
schema:deathPlace & place of death \\
schema:nationality & country of citizenship \\
schema:owns & owner of \\
schema:spouse & spouse \\
yago:studentOf & student of \\
yago:doctoralAdvisor & doctoral advisor \\
yago:playsIn & league or competition \\
yago:candidateIn & candidacy in election \\
yago:highestPoint & highest point \\
yago:lowestPoint & lowest point \\
yago:neighbors & located in or next to body of water, shares border with \\
yago:parentBody & parent astronomical body \\
yago:replaces & replaces \\
yago:capital & capital \\
yago:officialLanguage & official language \\
yago:flowsInto & outflows, mouth of the watercourse \\
yago:terminus & terminus location \\
schema:material & made from material \\
schema:manufacturer & developer, manufacturer \\
\bottomrule
\end{tabular}
    \caption{Mapping between YAGO relations and corresponding Wikidata relations used for dataset construction. Each YAGO relation is aligned to one or multiple Wikidata relations.}
    \label{tab:my_label}
\end{table}
